Are you SURE? Enhancing Multimodal Pretraining with Missing Modalities through Uncertainty Estimation

Multimodal learning has demonstrated incredible successes by integrating diverse data sources, yet it often relies on the availability of all modalities - an assumption that rarely holds in real-world applications. Pretrained multimodal models, while effective, struggle when confronted with small-scale and incomplete datasets (i.e., missing modalities), limiting their practical applicability. Previous studies on reconstructing missing modalities have overlooked the reconstruction's potential unreliability, which could compromise the quality of the final outputs. We present SURE (Scalable Uncertainty and Reconstruction Estimation), a novel framework that extends the capabilities of pretrained multimodal models by introducing latent space reconstruction and uncertainty estimation for both reconstructed modalities and downstream tasks. Our method is architecture-agnostic, reconstructs missing modalities, and delivers reliable uncertainty estimates, improving both interpretability and performance. SURE introduces a unique Pearson Correlation-based loss and applies statistical error propagation in deep networks for the first time, allowing precise quantification of uncertainties from missing data and model predictions. Extensive experiments across tasks such as sentiment analysis, genre classification, and action recognition show that SURE consistently achieves state-of-the-art performance, ensuring robust predictions even in the presence of incomplete data.

==> sections_edited/method_uncert_est_legacy.tex <==
\subsection{Distribution-free Uncertainty Estimation}
\label{sec:method_pearson_loss}
\textbf{Uncertainty Estimation Preliminaries.}
Bayesian deep learning models are capable of capturing uncertainty in their outputs. By maximizing a likelihood function, these models can optimize the network parameters to estimate the output distribution. This allows them to effectively capture aleatoric uncertainty, which arises from the inherent noise in the input data.
Specifically, for a given input $\textbf{x}_i$ from input domain $\mathcal{X}$, the corresponding model $\phi$ with parameters $\theta$ produces $\{\Tilde{\textbf{y}}_i, (\Tilde{\zeta}^1_i, \dots, \Tilde{\zeta}^k_i) \}$ (e.g. $:=\phi(\textbf{x}_i, \theta)$), which are parameters to specify the distribution $\mathcal{P}_{\textbf{Y}|\textbf{X}}$. The likelihood $\mathcal{L}(\theta, \mathcal{D}) := \prod_{i=1}^N p_{\textbf{Y}|\textbf{X}}(\textbf{y}_i; \{\Tilde{\textbf{y}}_i, \Tilde{\zeta}_i^1, \dots, \Tilde{\zeta}_i^k\})$ is then maximized to estimate the optimal parameters of the model. Additionally, the distribution $\mathcal{P}_{\textbf{Y}|\textbf{X}}$ is often chosen so that uncertainty can be estimated using a closed-form solution based on the model's estimated parameters. A common choice for this distribution is the heteroscedastic Gaussian \cite{upadhyay2022bayescap, wang2019aleatoric, NIPS2017_2650d608}, where $\phi(., \theta)$ predicts both the mean and variance. 
In this context, the predicted variance can be interpreted as the uncertainty of the prediction. The optimization problem then becomes:
\begin{equation}
\begin{aligned}
    \text{With } \{\Tilde{\textbf{y}}_i, \Tilde{\sigma}_i\} &:=\phi(\textbf{x}_i, \theta): \\
    \theta^* &=\underset{\theta}{\operatorname{argmax}} \prod_{i=1}^N \frac{1}{\sqrt{2 \pi \Tilde{\sigma}_i^2}} e^{-\frac{\left\|\Tilde{\textbf{y}}_i-\textbf{y}_i\right\|^2}{2 \Tilde{\sigma}_i^2}} \\
    &=\underset{\theta}{\operatorname{argmin}} \sum_{i=1}^N \frac{\left\|\Tilde{\mathbf{y}}_i-\mathbf{y}_i\right\|^2}{2 \Tilde{\sigma}_i^2}+\frac{\log \left(\Tilde{\sigma}_i^2\right)}{2}
    \label{eq:gaussian_mle}
\end{aligned}
\end{equation}
\begin{equation}
    \operatorname{Uncertainty}(\Tilde{\mathbf{y}}_i) = \Tilde{\sigma}^2_i.
\end{equation}
The closed-form solutions $\Tilde{\mathbf{y}}^i$ and $\Tilde{\sigma}^2_i$ for the problem in Equation \ref{eq:gaussian_mle} can be derived (the detailed process is shown in Appendix \ref{sec:app_gaussian_analyses}), with the final results as follows:
\begin{equation}
    % \begin{aligned}
        \Tilde{\mathbf{y}}_i^* = \mathbf{y}_i; \quad
        \Tilde{\sigma}^{2*}_i = \Tilde{\epsilon}^2_i \text{ where } \Tilde{\epsilon}^2_i := \left\|\Tilde{\mathbf{y}}_i-\mathbf{y}_i\right\|^2.
    % \end{aligned}
    \label{eq:gaussian_solution}
\end{equation}
The main drawback of this common approach is its reliance on assumptions about the true underlying distribution $\mathcal{P}_{\textbf{Y}|\textbf{X}}$, which may not hold true across all datasets and scenarios. Additionally, estimating uncertainty based specifically on a Gaussian assumption presents a further limitation due to the strict closed-form solution for $\Tilde{\sigma}^{2*}_i$ (Equation \ref{eq:gaussian_solution}). Ideally, the objective of Equation \ref{eq:gaussian_mle} would aim to learn a model capable of precisely approximating its own error $\Tilde{\epsilon}^2$. However, this becomes increasingly difficult as $\Tilde{\epsilon}^2 \rightarrow 0$, leading to unstable loss values and poorly defined gradients with respect to $\Tilde{\sigma}^{2*}_i$ (detailed analysis in Appendix \ref{sec:app_gaussian_analyses}). Consequently, achieving this strict objective through gradient-based optimization is highly challenging, if not impossible.

\textbf{Our method.} 
To overcome these limitations, we introduce a straightforward, distribution-free loss function centered on a more adaptable constraint for uncertainty: \emph{ensuring a strong correlation with error}. This loss function are employed to learn both reconstruction uncertainty as well as output uncertainty owing to model's inherent nature.
Specifically, we design our loss to learn the uncertainty $\Tilde{\sigma}^2$ by leveraging the Pearson Correlation Coefficient \cite{pcc} between $\Tilde{\sigma}^2$ and prediction error $\Tilde{\epsilon}^2$:
\begin{equation}
% \begin{gather*}
    \begin{aligned}
    &\mathcal{L}_{PCC}(\Tilde{\sigma}^2,\Tilde{\epsilon}^2) = 1 - r(\Tilde{\sigma}^2,\Tilde{\epsilon}^2); \\
    \text{ where } \\
    r(\Tilde{\sigma}^2, \Tilde{\epsilon}^2) &=\frac{\sum_{i=1}^N\left(\Tilde{\sigma}^2_i-\mu_{\sigma^2}\right)\left(\Tilde{\epsilon}^2_i-\mu_{\epsilon^2}\right)}{\sqrt{\sum_{i=1}^N\left(\Tilde{\sigma}^2_i-\mu_{\sigma^2}\right)^2} \sqrt{\sum_{i=1}^N\left(\Tilde{\epsilon}^2_i-\mu_{\epsilon^2}\right)^2}},  \\
    \mu_{\sigma^2} &= \frac{1}{N}\sum_{i=1}^N\Tilde{\sigma}^2_i, 
    \mu_{\epsilon^2} = \frac{1}{N}\sum_{i=1}^N\Tilde{\epsilon}^2_i, \Tilde{\epsilon}^2_i = \left\|\Tilde{\mathbf{y}}_i-\mathbf{y}_i\right\|^2,
    \end{aligned}
% \end{gather*}
\label{eq:pcc_loss}
\end{equation}
$N$ is the number of samples in one batch.
The Pearson correlation coefficient is essentially a normalized measure of covariance, ensuring that the result always falls within the range of -1 to 1. Consequently, $\mathcal{L}_{PCC}$ is constrained to a value between 0 and 2. A value of $\mathcal{L}_{PCC}=0$ indicates a perfect linear relationship where $\Tilde{\sigma}^2$ increases in tandem with $\Tilde{\epsilon}^2$, meaning the uncertainty accurately reflects the prediction error. Conversely, $\mathcal{L}_{PCC}=2$ implies an inverse relationship. 

In essence, $\mathcal{L}_{PCC}$ is equivalent to the Mean Squared Error (MSE) between squared error and uncertainty after standardization. Let $\bar{\sigma}_i^2 := \frac{\Tilde{\sigma}_i^2 - \mu_\sigma}{\sqrt{\frac{1}{N-1}\sum_{j=1}^{N}(\Tilde{\sigma}_j^2-\mu_{\sigma^2})^2}}$ and $\bar{\epsilon}_i^2 := \frac{\Tilde{\epsilon}_i^2 - \mu_{\epsilon^2}}{\sqrt{\frac{1}{N-1}\sum_{j=1}^{N}(\Tilde{\epsilon}_j^2-\mu_{\epsilon^2})^2}}$ be the standardized version of $\Tilde{\sigma}^2$ and $\Tilde{\epsilon}^2$ within a mini-batch, ensuring they have zero mean and unit variance. Given that $\frac{1}{N-1}\sum_i\left(\bar{\sigma}_i^2\right)^2=1$ and $\frac{1}{N-1} \sum_i\left(\bar{\epsilon}i^2\right)^2=1$, we have the derivation as follow:
\begin{equation}
\begin{aligned}
\frac{1}{2N} \sum_{i=1}^N\left(\bar{\sigma}^2_i-\bar{\epsilon}^2_i\right)^2 
 &=\frac{1}{2N}\left((2N-2)-2 \sum_{i=1}^N \bar{\sigma}^2_i \bar{\epsilon}^2_i\right) \\
 &=\frac{2N-2}{2N}(1-r(\Tilde{\sigma}^2, \Tilde{\epsilon}^2)) \approx \mathcal{L}_{PCC}.
\end{aligned}
\label{eq:mse_equivalent}
\end{equation}
This equivalence suggests that the loss function relaxes constraints on the magnitude of both $\Tilde{\epsilon}^2$ and $\Tilde{\sigma}^2$, while still enforcing a linear dependency between these two variables. 
After training with this loss function, the output uncertainty can be scaled using the mean and standard deviation of the training errors, allowing it to be approximately aligned with the actual testing error. 
Additionally, we later show in Appendix \ref{sec:app_gaussian_analyses} that our loss function promotes a more stable training process near the optimal solution, which is not the case for ordinary Gaussian NLL loss.

In addition to uncertainty estimation, other loss functions are employed to learn the reconstruction or output corresponding to the downstream task. The estimated uncertainty is aligned with the corresponding reconstruction or prediction error. For reconstruction or regression tasks, Mean Squared Error (MSE) is used to quantify the error, while for classification tasks, the error is represented by the cross-entropy loss value. For instance, final loss guiding SURE's reconstruction modules is:
\begin{equation}
    \mathcal{L}_{rec}^i(\Tilde{\mathbf{z}}^i, \Tilde{\sigma}^2_{z^i}) = \frac{1}{N}\sum\|\Tilde{\mathbf{z}}^i - \mathbf{z}^i\|^2 + \lambda \cdot \mathcal{L}_{PCC}(\Tilde{\sigma}^2_{z^i},\|\Tilde{\mathbf{z}}^i - \mathbf{z}^i\|^2).
\end{equation}
Here, the MSE term guides the learning of reconstructed $\Tilde{\mathbf{z}}^i$, while $\mathcal{L}_{PCC}$ ensures $\sigma^2$ reflects reconstruction error. $\lambda$ adjusts the contribution of each loss term. A similar loss function is applied to estimate the uncertainty of the output, accounting for the stochastic nature of pretrained models. In this context, the error $\Tilde{\epsilon}^2$ is defined as MSE for regression tasks or Cross Entropy for classification tasks. In parallel, we enhance the estimated output uncertainty by quantifying the uncertainty propagated from the reconstructed input, utilizing Error Propagation through the frozen pretrained network, as detailed in Section \ref{sec:method_error_propagation}.

==> sections_edited/reproducability.tex <==
\section*{Reproducability Statement}
% https://iclr.cc/Conferences/2024/AuthorGuide
% Reproducibility
% It is important that the work published in ICLR is reproducible. Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. For example, for novel models or algorithms, a link to a anonymous downloadable source code can be submitted as supplementary materials; for theoretical results, clear explanations of any assumptions and a complete proof of the claims can be included in the appendix; for any datasets used in the experiments, a complete description of the data processing steps can be provided in the supplementary materials. Each of the above are examples of things that can be referenced in the reproducibility statement. This optional reproducibility statement will not count toward the page limit, but should not be more than 1 page.
We have made extensive efforts to ensure the reproducibility of our work, focusing on several key areas:
\begin{itemize}
    \item Code Availability: The complete codebase for this work, including all models, training scripts, and evaluation procedures, is prepared. Upon acceptance, this code will be open-sourced and made publicly available on GitHub.
    \item Dataset Preparation: Detailed instructions for dataset setup, including any preprocessing steps and data splits used in our experiments, are provided in Section \ref{sec:experiments}, enabling other researchers to replicate our exact experimental conditions.
    \item Hardware and Hyperparameters: A comprehensive description of the hyperparameters used in our experiments, including optimization settings, the GPUs used, and other configuration details, is provided in Appendix  \ref{sec:app_compute}. 
    \item Architecture Transparency: Detailed descriptions of our model architectures are provided in Appendix \ref{sec:app_settings}, ensuring others can understand and reconstruct the models accurately. 
    \item Evaluation Metrics: The exact definitions of all evaluation metrics used are provided in Section \ref{sec:experiments} of the main paper.
\end{itemize}
By offering this comprehensive set of resources, we aim to facilitate the reproduction of our results by the research community. We believe that this level of transparency is crucial for advancing the field and supporting thorough validation and extension of our work.

==> tables/book.tex <==
\begin{table}[th]
\centering
\caption{Results of different approaches on Book Dataset.}
\label{tab:book}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lllcccc@{}}
\toprule
\textbf{}                                & \textbf{Model}                                                                   & \textbf{} & \multicolumn{1}{l}{\textbf{F1}}       & \multicolumn{1}{l}{\textbf{Acc}}      & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reconstruct\\ Uncertainty Corr\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Output\\ Uncertainty Corr\end{tabular}}} \\ \midrule
                                         &                                                                                  & Text      & 0.277                                 & 0.186                                 & -                                                                                                   & -                                                                                              \\
                                         &                                                                                  & Image     & 0.271                                 & 0.166                                 & -                                                                                                   & -                                                                                              \\
                                         & \multirow{-3}{*}{ActionMAE}                                                      & Full      & 0.35                                  & 0.311                                 & -                                                                                                   & -                                                                                              \\ \cmidrule(l){2-7} 
                                         &                                                                                  & Text      & 0.202                                 & 0.152                                 & -                                                                                                   & -                                                                                              \\
                                         &                                                                                  & Image     & 0.465                                 & 0.452                                 & -                                                                                                   & -                                                                                              \\
                                         & \multirow{-3}{*}{DiCMoR}                                                         & Full      & 0.467                                 & 0.454                                 & -                                                                                                   & -                                                                                              \\ \cmidrule(l){2-7} 
                                         &                                                                                  & Text      & 0.204                                 & 0.155                                 & -                                                                                                   & -                                                                                              \\
                                         &                                                                                  & Image     & 0.376                                 & 0.368                                 & -                                                                                                   & -                                                                                              \\
\multirow{-9}{*}{\rotatebox[origin=c]{90}{Modal Reconstruction}}   & \multirow{-3}{*}{IMDer}                                                          & Full      & 0.374                                 & 0.367                                 & -                                                                                                   & -                                                                                              \\ \midrule
                                         &                                                                                  & Text      & 0.676                                 & 0.665                                 & 0.137                                                                                               & 0.358                                                                                          \\
                                         &                                                                                  & Image     & 0.238                                 & 0.233                                 & 0.233                                                                                               & 0.349                                                                                          \\
                                         & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE +\\ Gaussian MLE\end{tabular}}  & Full      & \textcolor{blue}{0.685}          & 0.672                                 & -                                                                                                   & 0.468                                                                                          \\ \cmidrule(l){2-7} 
                                         &                                                                                  & Text      & 0.653                                 & 0.65                                  & 0.243                                                                                               & 0.174                                                                                          \\
                                         &                                                                                  & Image     & 0.491                                 & 0.466                                 & 0.334                                                                                               & 0.186                                                                                          \\
                                         & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ MC DropOut\end{tabular}}   & Full      & 0.669                                 & 0.658                                 & -                                                                                                   & 0.41                                                                                           \\ \cmidrule(l){2-7} 
                                         &                                                                                  & Text      & 0.682                                 & \textcolor{blue}{0.673}          & 0.128                                                                                               & 0.144                                                                                          \\
                                         &                                                                                  & Image     & 0.327                                 & 0.31                                  & 0.135                                                                                               & 0.214                                                                                          \\
\multirow{-9}{*}{\rotatebox[origin=c]{90}{Uncertainty Estimation}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ DeepEnsemble\end{tabular}} & Full      & 0.684                                 & \textcolor{blue}{0.673}          & -                                                                                                   & 0.227                                                                                          \\ \midrule
                                         &                                                                                  & Text      & 0.683                                 & 0.671                                 & \textcolor{blue}{0.637}                                                                        & 0.373                                                                                          \\
                                         &                                                                                  & Image     & 0.413                                 & 0.401                                 & {\color[HTML]{FF0000} \textbf{0.833}}                                                               & {\color[HTML]{FF0000} \textbf{0.481}}                                                          \\
                                         & \multirow{-3}{*}{SURE}                                                           & Full      & {\color[HTML]{FF0000} \textbf{0.696}} & {\color[HTML]{FF0000} \textbf{0.688}} & -                                                                                                   & \textcolor{blue}{0.474}                                                                   \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/mosi.tex <==
\begin{table}[th]
\centering
\caption{Results of different approaches on CMU-MOSI Dataset.}
\label{tab:mosi}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lllcccccc@{}}
\toprule
                                         & \textbf{Model}                                                                   & \textbf{} & \multicolumn{1}{l}{\textbf{MAE}}      & \multicolumn{1}{l}{\textbf{Corr}}     & \multicolumn{1}{l}{\textbf{F1}}       & \multicolumn{1}{l}{\textbf{Acc}}    & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reconstruct\\ Uncertainty Corr\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Output\\ Uncertainty Corr\end{tabular}}} \\ \midrule
                                         &                                                                                  & Text      & 1.106                                 & 0.506                                 & 0.717                                 & 0.724                               & -                                                         & -                                                    \\
                                         &                                                                                  & Audio     & 2.146                                 & 0.155                                 & 0.57                                  & 0.423                               & -                                                         & -                                                    \\
                                         & \multirow{-3}{*}{ActionMAE}                                                      & Full      & 1.005                                 & 0.517                                 & 0.719                                 & 0.725                               & -                                                         & -                                                    \\ \cmidrule(l){2-9} 
                                         &                                                                                  & Text      & 0.811                                 & 0.783                                 & 0.854                                 & 0.856                               & -                                                         & -                                                    \\
                                         &                                                                                  & Audio     & 1.227                                 & 0.427                                 & 0.57                                  & 0.585                               & -                                                         & -                                                    \\
                                         & \multirow{-3}{*}{DiCMoR}                                                         & Full      & 1.106                                 & 0.537                                 & 0.65                                  & 0.654                               & -                                                         & -                                                    \\ \cmidrule(l){2-9} 
                                         &                                                                                  & Text      & 0.707                                 & 0.797                                 & 0.846                                 & 0.846                               & -                                                         & -                                                    \\
                                         &                                                                                  & Audio     & 1.237                                 & 0.438                                 & 0.524                                 & 0.564                               & -                                                         & -                                                    \\
\multirow{-9}{*}{\rotatebox[origin=c]{90}{Modal Reconstruction}}   & \multirow{-3}{*}{IMDer}                                                          & Full      & 1.106                                 & 0.544                                 & 0.62                                  & 0.634                               & -                                                         & -                                                    \\ \midrule
                                         &                                                                                  & Text      & 0.589                                 & 0.866                                 & 0.88                                  & 0.879                               & 0.103                                                     & 0.067                                                \\
                                         &                                                                                  & Audio     & 1.133                                 & 0.53                                  & 0.676                                 & 0.678                               & 0.013                                                     & 0.032                                                \\
                                         & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ Gaussian MLE\end{tabular}} & Full      & \textcolor{red}{\textbf{0.581}} & \textcolor{red}{\textbf{0.871}} & 0.885                                 & 0.882                               & -                                                         & 0.059                                                \\ \cmidrule(l){2-9} 
                                         &                                                                                  & Text      & 0.63                                  & 0.858                                 & 0.877                                 & 0.876                               & 0.047                                                     & 0.013                                                \\
                                         &                                                                                  & Audio     & 1.153                                 & 0.556                                 & 0.686                                 & 0.684                               & 0.008                                                     & 0.009                                                \\
                                         & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ MC DropOut\end{tabular}}   & Full      & 0.622                                 & 0.865                                 & \textcolor{red}{\textbf{0.899}} & \textcolor{red}{\textbf{0.9}} & -                                                         & 0.13                                                 \\ \cmidrule(l){2-9} 
                                         &                                                                                  & Text      & 0.592                                 & 0.868                                 & 0.886                                 & 0.885                               & 0.062                                                     & 0.024                                                \\
                                         &                                                                                  & Audio     & 1.071                                 & 0.58                                  & 0.714                                 & 0.716                               & 0.031                                                     & 0.074                                                \\
\multirow{-9}{*}{\rotatebox[origin=c]{90}{Uncertainty Estimation}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ DeepEnsemble\end{tabular}} & Full      & \textcolor{blue}{0.582}          & \textcolor{red}{\textbf{0.871}} & 0.889                                 & 0.888                               & -                                                         & 0.082                                                \\ \midrule
                                         &                                                                                  & Text      & 0.602                                 & 0.865                                 & \textcolor{blue}{0.896}          & \textcolor{blue}{0.894}        & \textcolor{red}{\textbf{0.739}}                     & \textcolor{blue}{0.381}                         \\
                                         &                                                                                  & Audio     & 1.148                                 & 0.557                                 & 0.685                                 & 0.684                               & \textcolor{blue}{0.732}                              & 0.18                                                 \\
                                         & \multirow{-3}{*}{SURE}                                                           & Full      & 0.583                                 & 0.869                                 & 0.891                                 & 0.89                                & -                                                         & \textcolor{red}{\textbf{0.485}}                \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/utd_mhad.tex <==
\begin{table}[th]
\centering
\caption{Results of different approaches on UTD-MHAD Dataset. \duy{Reformat this for shorter height}}
\label{tab:utd_mhad}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lllcccc@{}}
\toprule
                                          & \textbf{Model}                                                                   &             & \multicolumn{1}{l}{\textbf{F1}} & \multicolumn{1}{l}{\textbf{Acc}}     & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Reconstruct \\ Uncertainty Corr\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}Output \\ Uncertainty Corr\end{tabular}}} \\ \midrule
                                          &                                                                                  & Video       & 0.044                           & 0.059                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Accel & 0.204                           & 0.231                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Gyro  & 0.303                           & 0.311                                & -                                                                                                    & -                                                                                               \\
                                          & \multirow{-4}{*}{ActionMAE}                                                      & Full        & 0.531                           & 0.537                                & -                                                                                                    & -                                                                                               \\ \cmidrule(l){2-7} 
                                          &                                                                                  & Video       & 0.069                           & 0.033                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Accel & 0.473                           & 0.408                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Gyro  & 0.52                            & 0.472                                & -                                                                                                    & -                                                                                               \\
                                          & \multirow{-4}{*}{DiCMoR}                                                         & Full        & 0.653                           & 0.636                                & -                                                                                                    & -                                                                                               \\ \cmidrule(l){2-7} 
                                          &                                                                                  & Video       & 0.089                           & 0.069                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Accel & 0.157                           & 0.158                                & -                                                                                                    & -                                                                                               \\
                                          &                                                                                  & Gyro  & 0.141                           & 0.145                                & -                                                                                                    & -                                                                                               \\
\multirow{-12}{*}{\rotatebox[origin=c]{90}{Modal Reconstruction}}   & \multirow{-4}{*}{IMDer}                                                          & Full        & 0.687                           & 0.689                                & -                                                                                                    & -                                                                                               \\ \midrule
                                          &                                                                                  & Video       & 0.116                           & 0.074                                & 0.166                                                                                                & 0.122                                                                                           \\
                                          &                                                                                  & Accel & 0.433                           & 0.381                                & 0.115                                                                                                & 0.476                                                                                           \\
                                          &                                                                                  & Gyro  & 0.468                           & 0.387                                & 0.056                                                                                                & 0.147                                                                                           \\
                                          & \multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ Gaussian MLE\end{tabular}} & Full        & 0.693                           & 0.651                                & -                                                                                                    & 0.292                                                                                           \\ \cmidrule(l){2-7} 
                                          &                                                                                  & Video       & 0.156                           & 0.09                                 & 0.122                                                                                                & 0.136                                                                                           \\
                                          &                                                                                  & Accel & 0.473                           & 0.404                                & 0.135                                                                                                & 0.486                                                                                           \\
                                          &                                                                                  & Gyro  & 0.595                           & 0.571                                & 0.171                                                                                                & 0.223                                                                                           \\
                                          & \multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ MC DropOut\end{tabular}}   & Full        & \textcolor{blue}{0.739}    & 0.718                                & -                                                                                                    & 0.512                                                                                           \\ \cmidrule(l){2-7} 
                                          &                                                                                  & Video       & 0.25                            & 0.207                                & 0.249                                                                                                & 0.126                                                                                           \\
                                          &                                                                                  & Accel & 0.468                           & 0.453                                & 0.175                                                                                                & 0.421                                                                                           \\
                                          &                                                                                  & Gyro  & 0.593                           & 0.604                                & 0.122                                                                                                & 0.436                                                                                           \\
\multirow{-12}{*}{\rotatebox[origin=c]{90}{Uncertainty Estimation}} & \multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}SURE + \\ DeepEnsemble\end{tabular}} & Full        & 0.737                           & \textcolor{blue}{0.735}         & -                                                                                                    & 0.481                                                                                           \\ \midrule
                                          &                                                                                  & Video       & 0.161                           & 0.121                                & \textcolor{red}{\textbf{0.878}}                                                                & 0.226                                                                                           \\
                                          &                                                                                  & Accel & 0.462                           & 0.431                                & 0.837                                                                                                & \textcolor{blue}{0.53}                                                                     \\
                                          &                                                                                  & Gyro  & 0.607                           & 0.59                                 & \textcolor{blue}{0.863}                                                                         & 0.306                                                                                           \\
                                          & \multirow{-4}{*}{SURE}                                                           & Full        & \textcolor{blue}{0.739}    & \textcolor{red}{\textbf{0.74}} & -                                                                                                    & \textcolor{red}{\textbf{0.568}}                                                           \\ \bottomrule
\end{tabular}
}
\end{table}
